Leveraging Self-Supervised Training for Unintentional Action Recognition

Unintentional actions are rare occurrences that are difficult to define precisely and that are highly dependent on the temporal context of the action. In this work, we explore such actions and seek to identify the points in videos where the actions transition from intentional to unintentional. We propose a multi-stage framework that exploits inherent biases such as motion speed, motion direction, and order to recognize unintentional actions. To enhance representations via self-supervised training for the task of unintentional action recognition we propose temporal transformations, called Temporal Transformations of Inherent Biases of Unintentional Actions (T2IBUA). The multi-stage approach models the temporal information on both the level of individual frames and full clips. These enhanced representations show strong performance for unintentional action recognition tasks. We provide an extensive ablation study of our framework and report results that significantly improve over the state-of-the-art.

==> tables/uar_ablation_backbone.tex <==
\begin{table}[H]
% \vspace{-4mm}
\centering
\small
\tabcolsep=0.1cm

\caption{Influence of different temporal encoders on UA classification task.$^{\star}$ indicates results copied from~\cite{epstein2019unint_actions}. FS: Fully-Supervised, SS: Self-Supervised pretraining.}
\begin{tabular}{ccc|c}
\toprule
Backbone & Pretrain Dataset & Pretraining & Accuracy \\
\midrule
R(2+1)D & Kinetics400 & FS & 53.2\\
ResNet3D-18$^{\star}$ & Oops! & SS & 53.4\\
ResNet3D-18$^{\star}$ & Kinetics700 & FS & 53.5\\
Ours (F2C2V) & Oops! & SS & \textbf{63.3}\\
\bottomrule
\end{tabular}
\label{table:uar_backbone}
% \vspace{-3mm}
\end{table}

==> tables/uar_ablation_crf_influence.tex <==
\begin{table}[t!]
\centering
\small
\tabcolsep=0.1cm
\caption{\fontsizenine{Ablation results: Influence of \tib and CRF layer on classification performance for two representations, pretrained ViT representation and R3D.}}
\label{table:uar_ablation_crf_influence}
\begin{tabular}{c|c|cc|cc}
\toprule
\multirow{2}{*}{\tib} & \multirow{2}{*}{CRF} & \multicolumn{2}{c}{ViT}  & \multicolumn{2}{c}{R3D} \\
& & F2C & F2C2V & F2C & F2C2V \\ 
\midrule
$-$ & $-$ &  60.9 & 69.6 & 59.3 & 65.6\\
\ding{52}&$-$ &  65.5 & 74.3 & 63.8 & 70.4 \\
\ding{52}&\ding{52} & 65.0 & \textbf{76.9} & 65.3 & \textbf{74.0}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/uar_ablation_rep_learning.tex <==
\begin{table}[]
\centering
\small
\tabcolsep=0.1cm
\begin{tabular}{c|cc}
\toprule
Pretraining & Acc. Frame & Acc. Clip\\
\midrule
\xmark & 60.9  & 74.5\\
\cmark & 65.0  & \textbf{76.9}\\
\bottomrule
\end{tabular}

\caption{Influence of the self-supervised pretraining on UA classification task.}
\label{table:uar_ablation_rep_learning}
% \vspace{-3mm}
\end{table}

==> tables/uar_ablation_stage1.tex <==
\begin{table}[H]
\centering
\small
\tabcolsep=0.1cm

\caption{Influence of Stage 1 on UA classification task. GAP denotes global average pooling operator instead of the $\mathfrak{T}_{frame}$ encoder. }

\begin{tabular}{c|c}
\toprule
Stage 1 & Accuracy \\
\midrule
$-$& 74.4\\
GAP & 75.0\\
$\mathfrak{T}_{frame}$ & \textbf{76.9}\\
\bottomrule
\end{tabular}
\label{table:uar_ablation_stage1}
% \vspace{-3mm}
\end{table}

==> tables/uar_ablation_trn_matrix.tex <==
\begin{table}[H]
\centering
\small
\tabcolsep=0.1cm
\caption{Influence of transition score matrix calculation method on UA classification task.}
\label{table:uar_ablation_trn_matrix}
\begin{tabular}{c|c}
\toprule
Calc. Method & Accuracy \\
\midrule
Binary & 74.8\\
Training split prior & 74.9\\
Trainable weights & \textbf{76.9}\\
\bottomrule
\end{tabular}
% \vspace{-3mm}
\end{table}

==> tables/uar_albation_trn_type.tex <==
\begin{table}[]
\centering
\small
\tabcolsep=0.1cm
\begin{tabular}{c|cc}
\toprule
\tib & F2C & F2C2V \\
\midrule
$-$& 60.9  & 73.2\\
Speed & 62.5  & 73.8\\
Direction & 63.3  & 75.1\\ %
All & \textbf{65.5} & \textbf{76.9}\\
\bottomrule
\end{tabular}

\caption{Influence of \tib groups on UA classification task for different stages of learning of the temporal encoder.}
\label{table:uar_ablation_trn_type}
% \vspace{-3mm}
\end{table}

==> tables/uar_sota_comparison_anticipation.tex <==

\begin{table}[]
\centering
\small
\tabcolsep=0.1cm
\begin{tabular}{c|ccc}
\toprule
& Accuracy after\\ 
Method & 1.5sec\\
\midrule
K700 Supervision & 59.7 \\
\midrule
Epstein \etal \cite{epstein2019unint_actions} & 56.7 \\
Ours (Frame) & 69.2 \\
Ours (Clip) & \textbf{78.1} \\

\bottomrule
\end{tabular}

\caption{Comparison of our approach to previous works for unintentional action localisation.}
\label{table:uar_sota_comparison_anticipation}
% \vspace{-3mm}
\end{table}

==> tables/uar_sota_comparison_localisation.tex <==

\begin{table}[]
\centering
\small
\tabcolsep=0.1cm
\begin{tabular}{c|ccc}
\toprule
& Accuracy within & Accuracy within\\ 
Method & 0.25sec & 1sec\\
\midrule
K700 Supervision & 46.7 & 75.9 \\
\midrule
Epstein \etal \cite{epstein2019unint_actions} & 36.6 & 65.3 \\
Ours (Frame) & \textbf{41.4} & \textbf{72.2} \\
Ours (Clip)& $\cdots$ & $\cdots$ \\

\bottomrule
\end{tabular}

\caption{Comparison of our approach to previous works for unintentional action localisation.}
\label{table:uar_sota_comparison_localisation}
% \vspace{-3mm}
\end{table}
